Performance Analysis of Deep Learning Workloads on Leading-edge Systems

This work examines the performance of leading-edge systems designed for machine learning computing, including the NVIDIA DGX-2, Amazon Web Services (AWS) P3, IBM Power System Accelerated Compute Server AC922, and a consumer-grade Exxact TensorEX TS4 GPU server. Representative deep learning workloads from the fields of computer vision and natural language processing are the focus of the analysis. Performance analysis is performed along with a number of important dimensions. Performance of the communication interconnects and large and high-throughput deep learning models are considered. Different potential use models for the systems as standalone and in the cloud also are examined. The effect of various optimization of the deep learning models and system configurations is included in the analysis.

==> src/apdx.tex <==
\appendix
% \section{CPU bottleneck}
% \subsection{Not Enough L1 Cache}
% {\ray L1 cache figure}
% \subsection{Data Loading Fluctuation}
% {\ray show the error bar of multiple runs.}
% \begin{figure*}
%   \centering
% \includegraphics[width=1.0\textwidth]{fig/dist_img_fp32}
% \caption{effects of number of processes per GPU}
% from left to right, aws-run1-j4, asw-run2-j4, dgx2-run1to5-j4, dgx2-j1, dgx2-j2, dgx2-j3, dgx2-j4, dgx2-j5, dgx2-j6
% \end{figure*}

\section{Changes}

\begin{itemize}
\item add new citation Tartan: Evaluating Modern GPU ...
\item add new citation Craig Tierney on NVSwitch.
\item remove $\Gamma$. in table. 
\item add annotations in the figure 2.
\item \cg{TODO} add std dev and discussion in results
\item fix the bias term in CNN operation computation analysis
\item add nccl-test perm-link.
\item explained the dashed grey lines in the caption
\item added warm-up phase is excluded from the statistics
\end{itemize}

\section{Additional Document}

\begin{itemize}
    \item \cg{TODO} add candidate new section to address mixed precision and fp32. on dgx2. to address 1) compare with existing results. 2) show the performance
    \item \cg{TODO} add p2p bandwidth section to help explain the topology difference.
    \item \cg{TODO} add plots with standard deviations of dgx2. show the runs are the same. 
    \item \cg{TODO} publish appendix either in arxiv or in BNL perm link
    \item \cg{TODO} tests for different $j$ on DGX-2
    \item \cg{TODO} different batch size?
\end{itemize}



==> src/results_bkup.tex <==
\section{Results: Case Studies}

\subsection{Communication Performance}\label{subsec:comm}
As shown in Section~\ref{subsec:hardware}, the leading-edge systems implement various 
direct high-bandwidth inter-device communication topologies based on NVLink.
The NVIDIA Collective Communication Library (NCCL)\footnote{https://github.com/NVIDIA/nccl}
provides MPI-like primitives
for multi-GPU and multi-node collective communications.  The library is
optimized for NVIDIA GPU devices to achieve high communication bandwidth over
NVLink and PCIe (when necessary).  NCCL supports collective
communication primitives, such as all-reduce,  all-gather, reduce-scatter, reduce and broadcast.

We present the performance of all-reduce and broadcast as the most relevant
communication kernels occurring in the benchmarks. 
We use the NCCL-tests\footnote{https://github.com/NVIDIA/nccl-tests} code developed by NVIDIA.
The results are presented as the bus bandwidth, a concept introduced by the
NCCL-tests.  Bus bandwidth is obtained by applying a formula to the measured
bandwidth ($message size / time$)\footnote{described in details
here: https://github.com/NVIDIA/nccl-tests/blob/master/doc/PERFORMANCE.md.}
Because the bus bandwidth reflects how optimally the hardware is used,
it provides a consistent and normalized way to compare the results with the theoretical peak
bandwidth for any communication primitives.

We varied the data size from 1MB to 1GB, which covers the communication
needs for synchronizing model parameters.  Each data point is averaged over 500
iterations except for the case of 16-GPU using two AWS-P3 which is averaged
over 50 iterations due to its slow inter-node Ethernet connection. 
Results are shown in Figure~\ref{fig:nccl}.
%The all-reduce NCCL kernel and broadcast  is primarily used in PyTorch distributed data-parallel
%training scenario, whereas the reduce and broadcast are used in PyTorch DataParallel module wrapper.
%At the end of every iteration, all model replicas need to
%synchronize by accumulating the gradients from other devices for each
%parameters of the model, thus an all-reduce communication with the ``sum'' operation. 

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\columnwidth}
        \centering
        \includegraphics[width=1.0\columnwidth]{fig/ALLREDUCE}
        \caption{\label{fig:allreduce} All-reduce}
        \vspace*{5mm}
    \end{subfigure}
    \begin{subfigure}[t]{1.0\columnwidth}
        \centering
        \includegraphics[width=1.0\columnwidth]{fig/BROADCAST}
        \caption{\label{fig:broadcast} Broadcast}
    \end{subfigure}
  \caption{\label{fig:nccl} Communication bus bandwidth.}
\end{figure}

DGX-2 achieves consistently 120GB/s for large message sizes, regardless of the
number of GPUs involved in the communication.  That is due to the link
bandwidth and contention (need discussion) properties of the NVSwitches
described in Section~\ref{subsec:hardware}.

% \sout{
% DGX-2 can achieve consistent 120GB/s for any number of the GPU devices. 
% As a reminder, DGX-2 connect all 16 GPUs with the cluster of 12 NVSwitches, Figure~\ref{fig:dgx2}.
% It does not matter how many GPUs are involved in the communication nor the type of collective communication.
% However, in most tested cases, the peak bandwidth of 150GB/s is not reached.
% The closest it can get is about 140GB/s when broadcasting messages from one GPU to the other (2GPUs), Figure~\ref{fig:broadcast}.
% }

AWS-P3 and DGX-1V yield very similar, if not exactly the same, results, 
as they share the same hybrid cube-mesh topology (see Figure~\ref{fig:dgx1}).
Due to the heterogeneity of this topology, the measured peak bandwidth depends on the devices involved in the communication.
In the case of 2 GPUs, the test uses device-0 and device-1, which are connected via a single NVLink providing 25GB/s 
theoretical unidirectional bandwidth. In the case of 4 GPUs, device-0-to-4 are in use and the NVLinks connecting to device-5-to7 
are not used. The observed bandwidth is 80GB/s. In the case of 8 GPUs, the DGX-1 surpasses the DGX-2 in all-reduce test
and with larger data package size (256MB) during broadcast test. We only had access to one DGX-1, therefore, the 16-GPU case 
was done on AWS-P3. The two AWS-p3dn nodes are connected via a 100Gbits/s multi-flow Ethernet connection. 
Our experimental setup in the AWS cloud allowed only a single flow (see Section~\ref{subsec:hardware}) with a peak bandwidth of 1.25GB/s.
The communication bandwidth in this case is clearly bottlenecked by the slow Ethernet connection.

IBM-AC922 utilizes half of the NVLinks for CPU-GPU communication (see Figure~\ref{fig:ac922}).
This leaves three NVLinks to connect device-0 and device-1.
In the case of 2 GPUs, the measured bus bandwidth 70GB/s is very close to the theoretical peak 75GB/s.
However, in the case of 4 GPUs, the bus bandwidth is reduced to about 30GB/s, matching the
theoretical SMP bus bandwidth 32GB/s connecting two Power9 CPUs.  \footnote{
At the moment of submitting this work, we are in the process of setting up the
other three IBM-AC922 machines.  We would like to update the results in future
(during revision).}

Our RTX system does not utilize NVLink technology and all 8 RTX 2080Ti GPUs are
connected through a PCIe bus.  Therefore, the communication bandwidth is
throttled down by the PCIe bus.  Despite its inferior communication
performance, we presents the RTX system as the baseline for other systems.


\subsection{Performance Analysis of Large Deep Learning Models}\label{subsec:largeDLM}
We measure the computation performance in terms of the model training throughput: 
the average number of training samples or \emph{instances} the system can process per second.
For every different combinations of systems, models, batch sizes and number of GPUs.
We measure the time intervals between consecutive iterations during training. 
For the computer vision deep learning models, each model ran 200 iterations.
For the BERT models, the reported throughput is averaged over training one epoch.

We are using the distributed data-parallel training with asynchronous data prefetching in single precision. 
Each GPU is associated with $j=4$ data-fetching CPU processes using CUDA Stream. 
Each GPU device holds a replica of the model. 
At the end of each iteration, all GPU synchronize their parameter gradients via a all-reduce NCCL operation. 
Then, they update the model parameters using the gradients individually.
The computer vision models are trained on the ILSVRC ImageNet data set (more than a million image files),
whereas the BERT models are fine-tuned on the task specific data sets, 
SWAG and SQuAD as introduced in Section~\ref{subsec:NLP}.


As the performance characteristics of the systems differ for different models, 
we group the models, such as ResNet101(152) and BERT,
as \emph{large} deep learning models,
and the models with high throughput, such as ResNet18(50) and AlexNet,
as \emph{high-throughput} deep learning models.  
We will discuss the results of the former in current sub-section, 
and latter in Section~\ref{subsec:smallDLM}.

%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%

\subsubsection{Scalability Study}
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1\columnwidth]{fig/SCALING-resnet50}
        \caption{\label{fig:scale-resnet50}ResNet50}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1\columnwidth]{fig/SCALING-resnet152}
        \caption{\label{fig:scale-resnet152}ResNet152}
    \vspace*{5mm}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1\columnwidth]{fig/SCALING-bert_swag}
        \caption{\label{fig:scale-bertswag}BERT-SWAG}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1\columnwidth]{fig/SCALING-bert_squad}
        \caption{\label{fig:scale-bertsquad}BERT-SQuAD}
    \end{subfigure}
  \caption{Scaling study on DGX2 and AWS-P3.
  The DGX2 shows a linear weak scaling up to 16 GPUs, whereas AWS-P3 up to 8 GPUs.
  }
\end{figure}



PyTorch on-node data parallel is the easiest
way to utilize multiple GPUs on a machine by simply wrapping the PyTorch
\texttt{Module} with a wrapper class called \texttt{DataParallel} {\ray toRef the PyTorch document}.

(Explain the communication patterns) 


%\subsection{Training on ImageNet Data using PyTorch Distributed Data Parallel}
\subsubsection{Effects of Batch Size on Performance}
[{\ray TODO}]

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-resnet101}
        \caption{\label{fig:gpumemresnet101} ResNet101}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-resnet152}
        \caption{\label{fig:gpumemresnet152} ResNet152}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-bert_swag}
        \caption{\label{fig:gpumembertswag} BERT-SWAG}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-bert_squad}
        \caption{\label{fig:gpumembertsquad} BERT-SQuAD}
    \end{subfigure}
    \caption{Performance under GPU Memory Limitation}
    {\ray TODO}
    The larger GPU memory will accommodate more training instances per iteration,
    or a larger batch size. To go through the same amount of instances, double 
    the batch size means halves the model synchronization (communication) costs.
    In all cases, a larger batch size will result a better throughput.
    DGX2, AWS-P3 and AC922 are all scaling well when communication is done inner-node.
    When using two nodes (16 GPUs), if we limit the GPU memory to 16GB, 
    AWS-P3 performs worse in training BERT-SQuAD comparing to using 8 GPUs.
    RTX uses the less powerful GPUs and scales reasonably well but not as good as NVLink-enabled systems.
\end{figure}


To optimize the data-parallel training scheme and to enable multi-node training, 
we need to use the fully-fledged distributed training. Every GPU node is paired with 
multiple CPU processes (4 in our tested case). The data are loaded and preprocessed 
asynchronously by CPU processes while the GPUs are in use. The inter-node and intra-node 
communications are managed by the NCCL back end. 

In the case of the AlexNet, when the computation is done on node (number of
GPUs less than 8), the DGX-2 and AWS-p3 have similar performance. However, when
working on 16 GPUs, AWS-p3 has to pay for the high cost of model
synchronization across the nodes.  The light computation workload (batch size
less than 128) makes the situation worse.  Light computation workload and fast
iterations also make the CPU processes constantly load and process data.  In
short, given the high communication costs and light computation workload, the
AlexNet is unsuitable for parallelization and cannot fully utilize the V100
GPUs. 

The case of the ResNet18 is more interesting. Since the model is only one sixth
of the AlexNet, the inter-node networking bottleneck of the AWS-p3 only shows
up when the workload is extremely light (batch size of 32). Interestingly, when
the batch size is large (more than 128 per GPU), the performance of AWS-p3 surpasses
DGX-2. This is due to the CPU cache bottle neck on DGX-2. Although the actual 
CPU clock speed of DGX-2 is higher than AWS-p3, the instructions per cycle (ipc) of DGX-2 
is much less than that of AWS-p3, 1.3~ipc vs 1.9~ipc. {\ray ToRef, see if we have space to 
show the ipc plot in appendix.} Again, like AlexNet, the light
computation workload of ResNet18 will not fully utilize the V100 GPUs.

For the larger models, such as ResNet50, ResNet101 and ResNet152, whose
computation workloads are heavier. If we fill the GPU memory as full as
possible (largest batch size), most of the GPU activities are spent on
computing rather than communication.  For example, on DGX-2 using all 16 GPUs
with batch size of 256, AlexNet spent about $80\%$ of GPU activities on
communication, whereas only about $4\%$ in the case of ResNet50. However, if we
only feed each GPU 32 instances per iteration, about $8\%$ of ResNet50's GPU
activities are on communication. Therefore, in general, we always want to fully
utilize the GPU memory. (and buy 32GB V100 instead of 16GB version.) The same
principle goes with the ResNet101 and ResNet152.  By assigning larger batch
size to fully utilize the GPU memory and reduce the needs of model
synchronization, the gap between AWS-p3 and DGX-2 are relatively small. The
ResNet50, due to its small model parameter size, makes the AWS-p3 a very
appealing option.  But when the model size is larger, like in ResNet152, the
penalty of narrow Ethernet bandwidth reveals. 

\subsection{Performance Analysis of High-throuput Deep Learning Models}\label{subsec:smallDLM}

The case of the ResNet18 is more interesting. Since the model is only one sixth
of the AlexNet, the inter-node networking bottleneck of the AWS-p3 only shows
up when the workload is extremely light (batch size of 32). Interestingly, when
the batch size is large (more than 128 per GPU), the performance of AWS-p3 surpasses
DGX-2. This is due to the CPU cache bottle neck on DGX-2. Although the actual 
CPU clock speed of DGX-2 is higher than AWS-p3, the instructions per cycle (ipc) of DGX-2 
is much less than that of AWS-p3, 1.3~ipc vs 1.9~ipc. {\ray ToRef, see if we have space to 
show the ipc plot in appendix.} Again, like AlexNet, the light
computation workload of ResNet18 will not fully utilize the V100 GPUs.

For the larger models, such as ResNet50, ResNet101 and ResNet152, whose
computation workloads are heavier. If we fill the GPU memory as full as
possible (largest batch size), most of the GPU activities are spent on
computing rather than communication.  For example, on DGX-2 using all 16 GPUs
with batch size of 256, AlexNet spent about $80\%$ of GPU activities on
communication, whereas only about $4\%$ in the case of ResNet50. However, if we
only feed each GPU 32 instances per iteration, about $8\%$ of ResNet50's GPU
activities are on communication. Therefore, in general, we always want to fully
utilize the GPU memory. (and buy 32GB V100 instead of 16GB version.) The same
principle goes with the ResNet101 and ResNet152.  By assigning larger batch
size to fully utilize the GPU memory and reduce the needs of model
synchronization, the gap between AWS-p3 and DGX-2 are relatively small. The
ResNet50, due to its small model parameter size, makes the AWS-p3 a very
appealing option.  But when the model size is larger, like in ResNet152, the
penalty of narrow Ethernet bandwidth reveals. 

\subsubsection{Scalability Study}

\subsubsection{Effects of Batch Size on Performance}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-alexnet}
        \caption{\label{fig:gpumemalexnet} AlexNet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-resnet18}
        \caption{\label{fig:gpumemresnet18} ResNet18}
    \end{subfigure}
    \caption{ Effects on Batch Size}
\end{figure}

\begin{figure}
  \begin{subfigure}[t]{0.49\columnwidth}
      \includegraphics[width=1.0\columnwidth]{fig/core_speed}
      \caption{\label{fig:corespeed} CPU Core Speed}
  \end{subfigure}
  \begin{subfigure}[t]{0.49\columnwidth}
      \includegraphics[width=1.0\columnwidth]{fig/ipc}
      \caption{\label{fig:ipc} Instructions per Cycle}
  \end{subfigure}
  \caption{Performance of smaller models}
\end{figure}


\subsection{Scaling of the Centralized Data Parallel Scheme}\label{subsec:cdp}
[{\ray TODO}]

\begin{figure}[ht]
  \centering
  %\includegraphics[width=\textwidth]{fig/barplot_bert}
  \includegraphics[width=1.0\columnwidth]{fig/CENTRAL-DP}
  \caption{\label{fig:central} Centralized vs Distributed: comparing two data parallel schemes}
  The PyTorch easy-to-use centralized data parallel scheme performs well when two GPUs are in use. 
  The lighter color indicates the centralized data parallel scheme.
\end{figure}




==> src/results_old.tex <==
\section{Results: Case Studies}

\subsection{Collective Communication: NCCL}


\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{fig/NCCLBW}
  \caption{\label{fig:nccl} NCCL communication bandwidth.}
  [{\ray Suitable for 2 systems}]
  %\Description{ [{\ray TODO}]}
\end{figure}


\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{fig/ALLREDUCE}
  \caption{\label{fig:allreduce} NCCL communication bandwidth.}
  [{\ray Suitable for more than 2 systems}]
  %\Description{ [{\ray TODO}]}
\end{figure}
The NVIDIA Collective Communication Library (NCCL) provides MPI-like primitives
for multi-GPU and multi-node collective communications.  The library is
optimized for NVIDIA GPU devices to achieve high communication bandwidth over
PCIe and NVLink (when available).  Among all the supported collective
communication primitives, such as all-reduce, broadcast and all-gather, the
all-reduce NCCL kernel is used most frequently in a distributed data-parallel
training scenario.  At the end of every iteration, all model replicas need to
synchronize by accumulating the gradients from other devices for each
parameters of the model, thus an all-reduce communication with the ``sum'' operation. 

We investigate the physical bidirectional bandwidth of all the systems we have tested.

\subsubsection*{RTX-DevBox} we tested does not have inter-node connections. All
the communications are passing through the PCIe bus.

\subsubsection*{AWS-p3dn} (DGX-I) links GPU devices via NVLink in a hybrid
grid-mesh topology, Figure~{\ray ToRef}.  Due to the heterogeneity of this
topology, the maximum bandwidth will depend on the devices involved in the
communication. Namely, to reach the maximum bandwidth (all six NVLink outlets
of a V100 GPU device), all eight GPU devices must be included in the
communication. The two-node AWS-p3dn setup we tested establish a 10Gbits/s
single-flow (100Gbits/s multi-flow) communication via an Ethernet connection.
Therefore, the 16-GPU case is bounded by the Ethernet bandwidth, about 1GB/s.

\subsubsection*{DGX-2} links all 16 GPUs through a cluster of NVSwitches, Figure~{\ray ToRef}.
As the topology is homogeneous and all six of the NVLink ports of a Tesla V100 GPU are used,
the tested maximum bandwidth of 120GB/s can always be reached no mater how many
devices are involved in the collective communication.  

The results are shown in Figure~\ref{fig:nccl}.

(We first investigate the physical limitations of the inter-device 
All-reduce (and Broadcast nccl) kernels are used in distributed learning.) 
[{\ray TODO}]


\subsection{Training on ImageNet Data using PyTorch On-node Data Parallel}
[{\ray TODO}]


\begin{figure*}[ht]
  \centering
  %\includegraphics[width=\linewidth]{fig/dp_img_fp32}
  \includegraphics[width=0.8\linewidth]{fig/IMGNETDP}
  \caption{\label{fig:imgdp} On-node Data Parallel Using NCCL(?).}
  [{\ray TODO}]
  %  \Description{ [{\ray TODO}]}
\end{figure*}


PyTorch on-node data parallel is the easiest
way to utilize multiple GPUs on a machine by simply wrapping the PyTorch
\texttt{Module} with a wrapper class called \texttt{DataParallel} {\ray toRef the PyTorch document}.

(Explain the communication patterns) 


\subsection{Training on ImageNet Data using PyTorch Distributed Data Parallel}
[{\ray TODO}]

\begin{figure*}[ht]
  \centering
  %\includegraphics[width=\linewidth]{fig/dist_img_fp32}
  \includegraphics[width=0.8\linewidth]{fig/IMGNETDIST}
  \caption{\label{fig:imgdist} Distributed Data Parallel Using NCCL}
  [{\ray TODO}]
  %\Description{ [{\ray TODO}]}
\end{figure*}

\begin{figure*}[ht]
  \centering
  %\includegraphics[width=\linewidth]{fig/dist_img_fp32}
  \includegraphics[width=0.8\linewidth]{fig/IMGNETDISTlog}
  \caption{\label{fig:imgdistlog} Distributed Data Parallel Using NCCL}
  [{\ray TODO}]
  %\Description{ [{\ray TODO}]}
\end{figure*}

To optimize the data-parallel training scheme and to enable multi-node training, 
we need to use the fully-fledged distributed training. Every GPU node is paired with 
multiple CPU processes (4 in our tested case). The data are loaded and preprocessed 
asynchronously by CPU processes while the GPUs are in use. The inter-node and intra-node 
communications are managed by the NCCL back end. 

In the case of the AlexNet, when the computation is done on node (number of
GPUs less than 8), the DGX-2 and AWS-p3 have similar performance. However, when
working on 16 GPUs, AWS-p3 has to pay for the high cost of model
synchronization across the nodes.  The light computation workload (batch size
less than 128) makes the situation worse.  Light computation workload and fast
iterations also make the CPU processes constantly load and process data.  In
short, given the high communication costs and light computation workload, the
AlexNet is unsuitable for parallelization and cannot fully utilize the V100
GPUs. 

The case of the ResNet18 is more interesting. Since the model is only one sixth
of the AlexNet, the inter-node networking bottleneck of the AWS-p3 only shows
up when the workload is extremely light (batch size of 32). Interestingly, when
the batch size is large (more than 128 per GPU), the performance of AWS-p3 surpasses
DGX-2. This is due to the CPU cache bottle neck on DGX-2. Although the actual 
CPU clock speed of DGX-2 is higher than AWS-p3, the instructions per cycle (ipc) of DGX-2 
is much less than that of AWS-p3, 1.3~ipc vs 1.9~ipc. {\ray ToRef, see if we have space to 
show the ipc plot in appendix.} Again, like AlexNet, the light
computation workload of ResNet18 will not fully utilize the V100 GPUs.

For the larger models, such as ResNet50, ResNet101 and ResNet152, whose
computation workloads are heavier. If we fill the GPU memory as full as
possible (largest batch size), most of the GPU activities are spent on
computing rather than communication.  For example, on DGX-2 using all 16 GPUs
with batch size of 256, AlexNet spent about $80\%$ of GPU activities on
communication, whereas only about $4\%$ in the case of ResNet50. However, if we
only feed each GPU 32 instances per iteration, about $8\%$ of ResNet50's GPU
activities are on communication. Therefore, in general, we always want to fully
utilize the GPU memory. (and buy 32GB V100 instead of 16GB version.) The same
principle goes with the ResNet101 and ResNet152.  By assigning larger batch
size to fully utilize the GPU memory and reduce the needs of model
synchronization, the gap between AWS-p3 and DGX-2 are relatively small. The
ResNet50, due to its small model parameter size, makes the AWS-p3 a very
appealing option.  But when the model size is larger, like in ResNet152, the
penalty of narrow Ethernet bandwidth reveals. 

\subsection{Fine-tuning BERT models using Distributed Data Parallel}
[{\ray TODO}]

\begin{figure*}[ht]
  \centering
  %\includegraphics[width=\textwidth]{fig/barplot_bert}
  \includegraphics[width=0.7\textwidth]{fig/BERT}
  \caption{\label{fig:bert} Fine-tuning BERT models using distributed data parallel }
  [{\ray TODO}]
  %\Description{ [{\ray TODO}]}
\end{figure*}

\begin{figure*}[ht]
  \centering
  %\includegraphics[width=\textwidth]{fig/barplot_bert}
  \includegraphics[width=0.7\textwidth]{fig/BERTlog}
  \caption{\label{fig:bertlog} Fine-tuning BERT models using distributed data parallel }
  [{\ray TODO}]
  %\Description{ [{\ray TODO}]}
\end{figure*}

The case of the ResNet18 is more interesting. Since the model is only one sixth
of the AlexNet, the inter-node networking bottleneck of the AWS-p3 only shows
up when the workload is extremely light (batch size of 32). Interestingly, when
the batch size is large (more than 128 per GPU), the performance of AWS-p3 surpasses
DGX-2. This is due to the CPU cache bottle neck on DGX-2. Although the actual 
CPU clock speed of DGX-2 is higher than AWS-p3, the instructions per cycle (ipc) of DGX-2 
is much less than that of AWS-p3, 1.3~ipc vs 1.9~ipc. {\ray ToRef, see if we have space to 
show the ipc plot in appendix.} Again, like AlexNet, the light
computation workload of ResNet18 will not fully utilize the V100 GPUs.

For the larger models, such as ResNet50, ResNet101 and ResNet152, whose
computation workloads are heavier. If we fill the GPU memory as full as
possible (largest batch size), most of the GPU activities are spent on
computing rather than communication.  For example, on DGX-2 using all 16 GPUs
with batch size of 256, AlexNet spent about $80\%$ of GPU activities on
communication, whereas only about $4\%$ in the case of ResNet50. However, if we
only feed each GPU 32 instances per iteration, about $8\%$ of ResNet50's GPU
activities are on communication. Therefore, in general, we always want to fully
utilize the GPU memory. (and buy 32GB V100 instead of 16GB version.) The same
principle goes with the ResNet101 and ResNet152.  By assigning larger batch
size to fully utilize the GPU memory and reduce the needs of model
synchronization, the gap between AWS-p3 and DGX-2 are relatively small. The
ResNet50, due to its small model parameter size, makes the AWS-p3 a very
appealing option.  But when the model size is larger, like in ResNet152, the
penalty of narrow Ethernet bandwidth reveals. 


==> src/results_ray.tex <==
\section{Results: Case Studies}

\subsection{Communication Performance}\label{subsec:comm}
As shown in Section~\ref{subsec:hardware}, the leading-edge systems implement various 
direct high-bandwidth inter-device communication topologies based on NVLink.
The NVIDIA Collective Communication Library (NCCL)\footnote{https://github.com/NVIDIA/nccl}
provides MPI-like primitives
for multi-GPU and multi-node collective communications.  The library is
optimized for NVIDIA GPU devices to achieve high communication bandwidth over
NVLink and PCIe (when necessary).  NCCL supports collective
communication primitives, such as all-reduce,  all-gather, reduce-scatter, reduce and broadcast.

We present the performance of all-reduce and broadcast as the most relevant
communication kernels occurring in the benchmarks. 
We use the NCCL-tests\footnote{https://github.com/NVIDIA/nccl-tests} code developed by NVIDIA.
The results are presented as the bus bandwidth, a concept introduced by the
NCCL-tests.  Bus bandwidth is obtained by applying a formula to the measured
bandwidth ($message size / time$)\footnote{described in details
here: https://github.com/NVIDIA/nccl-tests/blob/master/doc/PERFORMANCE.md.}
Because the bus bandwidth reflects how optimally the hardware is used,
it provides a consistent and normalized way to compare the results with the theoretical peak
bandwidth for any communication primitives.

We varied the data size from 1MB to 1GB, which covers the communication
needs for synchronizing model parameters.  Each data point is averaged over 500
iterations except for the case of 16-GPU using two AWS P3 which is averaged
over 50 iterations due to its slow inter-node Ethernet connection. 
Results are shown in Figure~\ref{fig:nccl}.
%The all-reduce NCCL kernel and broadcast  is primarily used in PyTorch distributed data-parallel
%training scenario, whereas the reduce and broadcast are used in PyTorch DataParallel module wrapper.
%At the end of every iteration, all model replicas need to
%synchronize by accumulating the gradients from other devices for each
%parameters of the model, thus an all-reduce communication with the ``sum'' operation. 

\begin{figure}[ht]
    \begin{subfigure}[t]{1.0\columnwidth}
        \centering
        \includegraphics[width=1.0\columnwidth]{fig/ALLREDUCE}
        \caption{\label{fig:allreduce} All-reduce}
        \vspace*{5mm}
    \end{subfigure}
    \begin{subfigure}[t]{1.0\columnwidth}
        \centering
        \includegraphics[width=1.0\columnwidth]{fig/BROADCAST}
        \caption{\label{fig:broadcast} Broadcast}
    \end{subfigure}
  \caption{\label{fig:nccl} Communication bus bandwidth.}
\end{figure}

DGX-2 achieves consistently 120GB/s for large message sizes, regardless of the
number of GPUs involved in the communication.  That is due to the link
bandwidth and contention (need discussion) properties of the NVSwitches
described in Section~\ref{subsec:hardware}.

% \sout{
% DGX-2 can achieve consistent 120GB/s for any number of the GPU devices. 
% As a reminder, DGX-2 connect all 16 GPUs with the cluster of 12 NVSwitches, Figure~\ref{fig:dgx2}.
% It does not matter how many GPUs are involved in the communication nor the type of collective communication.
% However, in most tested cases, the peak bandwidth of 150GB/s is not reached.
% The closest it can get is about 140GB/s when broadcasting messages from one GPU to the other (2GPUs), Figure~\ref{fig:broadcast}.
% }

AWS P3 and DGX-1V yield very similar, if not exactly the same, results, 
as they share the same hybrid cube-mesh topology (see Figure~\ref{fig:dgx1}).
Due to the heterogeneity of this topology, the measured peak bandwidth depends on the devices involved in the communication.
In the case of 2 GPUs, the test uses device-0 and device-1, which are connected via a single NVLink providing 25GB/s 
theoretical unidirectional bandwidth. In the case of 4 GPUs, device-0-to-4 are in use and the NVLinks connecting to device-5-to7 
are not used. The observed bandwidth is 80GB/s. In the case of 8 GPUs, the DGX-1 surpasses the DGX-2 in all-reduce test
and with larger data package size (256MB) during broadcast test. We only had access to one DGX-1, therefore, the 16-GPU case 
was done on AWS P3. The two AWS-p3dn nodes are connected via a 100Gbits/s multi-flow Ethernet connection. 
Our experimental setup in the AWS cloud allowed only a single flow (see Section~\ref{subsec:hardware}) with a peak bandwidth of 1.25GB/s.
The communication bandwidth in this case is clearly bottlenecked by the slow Ethernet connection.

IBM-AC922 utilizes half of the NVLinks for CPU-GPU communication (see Figure~\ref{fig:ac922}).
This leaves three NVLinks to connect device-0 and device-1.
In the case of 2 GPUs, the measured bus bandwidth 70GB/s is very close to the theoretical peak 75GB/s.
However, in the case of 4 GPUs, the bus bandwidth is reduced to about 30GB/s, matching the
theoretical SMP bus bandwidth 32GB/s connecting two Power9 CPUs.  \footnote{
At the moment of submitting this work, we are in the process of setting up the
other three IBM-AC922 machines.  We would like to update the results in future
(during revision).}

Our RTX system does not utilize NVLink technology and all 8 RTX 2080Ti GPUs are
connected through a PCIe bus.  Therefore, the communication bandwidth is
throttled down by the PCIe bus.  Despite its inferior communication
performance, we presents the RTX system as the baseline for other systems.


\subsection{Performance Analysis of Large Deep Learning Models}\label{subsec:largeDLM}
We measure the computation performance in terms of the model training throughput: 
the average number of training samples or \emph{instances} the system can process per second.
For every different combinations of models, batch sizes and number of GPUs,
we measure the time intervals between consecutive iterations during training. 
For the computer vision deep learning models, each model ran 200 iterations.
For the BERT models, the reported throughput is averaged over one training 
epoch\footnote{one epoch is defined as going through the entire data set once.}
All the models are represented in single precision (FP32).

We are using the distributed data-parallel training with asynchronous data prefetching.
Each GPU is associated with $j$ ($j=4$ in this test) data-fetching CPU processes using CUDA Stream. 
This allows data to be loaded and preprocessed asynchronously by CPU processes while the GPUs are in use. 
Every GPU device holds a replica of the model and applies the model on different batches of data.
At the end of each iteration, all GPUs synchronize their parameter gradients via a all-reduce NCCL operation. 
The NCCL supports both inter-node and intra-node communication.
Then, all model replica individually update their parameters using the gradients.
The computer vision models are trained on the ILSVRC ImageNet data set.
The ILSVRC ImageNet contains more than a million image files.
The BERT models are fine-tuned on the task specific data sets, 
SWAG and SQuAD as introduced in Section~\ref{subsec:nlp}.

As the performance characteristics of the systems differ for different models, 
we group the models, such as ResNet101(152) and BERT,
as \emph{large} deep learning models,
and the models with high throughput, such as ResNet18(50) and AlexNet,
as \emph{high-throughput} deep learning models.  
We will discuss the results of the former in the current sub-section, 
and latter in Section~\ref{subsec:smallDLM}.

%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%

\subsubsection{Scalability Study}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1\columnwidth]{fig/SCALING-resnet101}
        \caption{\label{fig:scale-resnet50}ResNet101}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1\columnwidth]{fig/SCALING-resnet152}
        \caption{\label{fig:scale-resnet152}ResNet152}
    \vspace*{5mm}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1\columnwidth]{fig/SCALING-bert_swag}
        \caption{\label{fig:scale-bertswag}BERT-SWAG}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1\columnwidth]{fig/SCALING-bert_squad}
        \caption{\label{fig:scale-bertsquad}BERT-SQuAD}
    \end{subfigure}
    \caption{\label{fig:scale-LDM}Scaling study on DGX2 and AWS P3.
      The DGX2 shows a linear scaling up to 16 GPUs, whereas AWS P3 up to 8 GPUs.
  }
\end{figure}

We first study the scaling property of large deep learning models,
such as ResNet101, ResNet152, BERT-SWAG and BERT-SQuAD, Figure~\ref{fig:scale-LDM}.
As the amount of communication for synchronization depends on the number of model parameters, not the batch size,
To achieve the best posible scaling results, we choose the largest 
batch size we can fit into the 32GB memory of V100 GPUs,
specifically: 128 per GPU in the case of ResNet101 and ResNet152, 64 of
BERT-SWAG and 32 of BERT-SQuAD.  

DGX-2 and AWS P3 have similar performance upto 8 GPUs across all four models.
This is expected as both systems have the same V100 GPUs and connected via
high-bandwidth (120GB/s) NVLinks.  However, when 16 GPUs are in use, two AWS
P3s communicate through a relatively slow Ethernet connection (about 1GB/s).
The difference in performance reveals, espeically in BERT models where the number 
of parameters is large, Figure~\ref{fig:scale-bertswag}~and~\ref{fig:scale-bertsquad}.



\subsubsection{Effects of Batch Size on Performance}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-resnet101}
        \caption{\label{fig:gpumemresnet101} ResNet101}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-resnet152}
        \caption{\label{fig:gpumemresnet152} ResNet152}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-bert_swag}
        \caption{\label{fig:gpumembertswag} BERT-SWAG}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-bert_squad}
        \caption{\label{fig:gpumembertsquad} BERT-SQuAD}
    \end{subfigure}
    \caption{Effects of Batch Size on Performance}
\end{figure}

The larger GPU memory will accommodate more training instances per iteration,
or a larger batch size. To go through the same amount of instances, double 
the batch size means halves the model synchronization (communication) costs.
In all cases, a larger batch size will result a better throughput.
DGX2, AWS-P3 and AC922 are all scaling well when communication is done inner-node.
When using two nodes (16 GPUs), if we limit the GPU memory to 16GB, 
AWS-P3 performs worse in training BERT-SQuAD comparing to using 8 GPUs.
RTX uses the less powerful GPUs and scales reasonably well but not as good as NVLink-enabled systems.



%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%
%%%==========================================================%%%

\subsection{Performance Analysis of High-throuput Deep Learning Models}\label{subsec:smallDLM}
In the case of the AlexNet, when the computation is done on node (number of
GPUs less than 8), the DGX-2 and AWS-p3 have similar performance. However, when
working on 16 GPUs, AWS-p3 has to pay for the high cost of model
synchronization across the nodes.  The light computation workload (batch size
less than 128) makes the situation worse.  Light computation workload and fast
iterations also make the CPU processes constantly load and process data.  In
short, given the high communication costs and light computation workload, the
AlexNet is unsuitable for parallelization and cannot fully utilize the V100
GPUs. 

The case of the ResNet18 is more interesting. Since the model is only one sixth
of the AlexNet, the inter-node networking bottleneck of the AWS-p3 only shows
up when the workload is extremely light (batch size of 32). Interestingly, when
the batch size is large (more than 128 per GPU), the performance of AWS-p3 surpasses
DGX-2. This is due to the CPU cache bottle neck on DGX-2. Although the actual 
CPU clock speed of DGX-2 is higher than AWS-p3, the instructions per cycle (ipc) of DGX-2 
is much less than that of AWS-p3, 1.3~ipc vs 1.9~ipc. {\ray ToRef, see if we have space to 
show the ipc plot in appendix.} Again, like AlexNet, the light
computation workload of ResNet18 will not fully utilize the V100 GPUs.

For example, on DGX-2 using all 16 GPUs
with batch size of 256, AlexNet spent about $80\%$ of GPU activities on
communication, whereas only about $4\%$ in the case of ResNet50. However, if we
only feed each GPU 32 instances per iteration, about $8\%$ of ResNet50's GPU
activities are on communication. Therefore, in general, we always want to fully
utilize the GPU memory. (and buy 32GB V100 instead of 16GB version.) The same
principle goes with the ResNet101 and ResNet152.  By assigning larger batch
size to fully utilize the GPU memory and reduce the needs of model
synchronization, the gap between AWS-p3 and DGX-2 are relatively small. The
ResNet50, due to its small model parameter size, makes the AWS-p3 a very
appealing option.  But when the model size is larger, like in ResNet152, the
penalty of narrow Ethernet bandwidth reveals. 


\subsubsection{Scalability Study}

\subsubsection{Effects of Batch Size on Performance}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-alexnet}
        \caption{\label{fig:gpumemalexnet} AlexNet}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
        \includegraphics[width=1.0\columnwidth]{fig/GPUMEM-resnet18}
        \caption{\label{fig:gpumemresnet18} ResNet18}
    \end{subfigure}
    \caption{ Effects on Batch Size}
\end{figure}

\begin{figure}
  \begin{subfigure}[t]{0.49\columnwidth}
      \includegraphics[width=1.0\columnwidth]{fig/core_speed}
      \caption{\label{fig:corespeed} CPU Core Speed}
  \end{subfigure}
  \begin{subfigure}[t]{0.49\columnwidth}
      \includegraphics[width=1.0\columnwidth]{fig/ipc}
      \caption{\label{fig:ipc} Instructions per Cycle}
  \end{subfigure}
  \caption{Performance of smaller models}
\end{figure}


\subsection{Scaling of the Centralized Data Parallel Scheme}\label{subsec:cdp}
[{\ray TODO}]

PyTorch on-node data parallel is the easiest
way to utilize multiple GPUs on a machine by simply wrapping the PyTorch
\texttt{Module} with a wrapper class called \texttt{DataParallel} {\ray toRef the PyTorch document}.

(Explain the communication patterns) 

\begin{figure}[ht]
  \centering
  %\includegraphics[width=\textwidth]{fig/barplot_bert}
  \includegraphics[width=1.0\columnwidth]{fig/CENTRAL-DP}
  \caption{\label{fig:central} Centralized vs Distributed: comparing two data parallel schemes}
  The PyTorch easy-to-use centralized data parallel scheme performs well when two GPUs are in use. 
  The lighter color indicates the centralized data parallel scheme.
\end{figure}



